When Can We Answer Queries Using Result-Bounded Data Interfaces?

We consider answering queries on data available through access methods, that provide lookup access to the tuples matching a given binding. Such interfaces are common on the Web; further, they often have bounds on how many results they can return, e.g., because of pagination or rate limits. We thus study result-bounded methods, which may return only a limited number of tuples. We study how to decide if a query is answerable using result-bounded methods, i.e., how to compute a plan that returns all answers to the query using the methods, assuming that the underlying data satisfies some integrity constraints. We first show how to reduce answerability to a query containment problem with constraints. Second, we show "schema simplification" theorems describing when and how result-bounded services can be used. Finally, we use these theorems to give decidability and complexity results about answerability for common constraint classes.

==> conseqch.tex <==
As we can restrict to a bound of~$1$, for schemas consisting of guarded TGDs,
we can use Proposition~\ref{prop:elimupper} and obtain an entailment for~$\amd$
which only involves guarded TGDs.
Thus:
\begin{thm} \label{thm:guarded} For a schema involving only guarded TGDs,
  monotone answerability is decidable in~$\twoexp$.
\end{thm}
The same proof applies to the \emph{Frontier-guarded TGDs} of \cite{baget2010walking}.



==> full-finite.tex <==
\subsection{Extensions to the Finite Variants} \label{subsec:fullfinite}
Recall that our notion of RA answerability considers equivalence of the plan
and the query  over all instances, finite and infinite. A stronger notion of answerability
would be \emph{finite RA answerability}: there is a plan that is equivalent to the query over all instances.

We now sketch the argument that \emph{all of the results stated in this appendix extend to the finite case}



==> organ.tex <==

\paragraph{Paper structure.} Section~\ref{sec:prelims}
  presents our model of accesses and plans over services, and
gives the definition of a query being answerable by a plan.
Section~\ref{sec:reduce} describes the reduction
of answerability to query containment which we use in our later results.
Section~\ref{sec:simplify}
presents our schema simplification results,
while Section~\ref{sec:complexity}
 applies them
to show decidability of the answerability problem. This analysis is extended to
more expressive constraints in Sections~\ref{sec:simplifychoice}
and~\ref{sec:complexitychoice}.
The paper closes in Section~\ref{sec:conc} with conclusions and discussion of future work.
Some extensions of the main results in the paper  are deferred to the appendix.



==> widthreduce.tex <==

\paragraph{Concluding the proof.}
We now apply the machinery to show our result on monotone answerability on
bounded-width $\incd$s, concluding the section.

\begin{proof}[Proof sketch of Theorem~\ref{thm:npidsbounds}]
  We only show the case without result bounds here; the case with
  result bounds is shown in Appendix~\ref{apx:npidsbounds}.
  The lower bound already holds without result bounds or constraints~\cite{access2},
  so we focus on $\np$-membership.

In the absence of result bounds, the~$\amd$ query containment problem
$Q \subseteq_\Gamma Q'$ has the following simpler form~\cite{ustods,thebook}:
$\Gamma$ contains $\Sigma, \Sigma'$ and\\[.2em]
  \null\hfill$\left(\bigwedge_i \accessible(x_i)\right) \wedge
  R(\vec x, \vec y) \rightarrow R'(\vec x, \vec y) \wedge \bigwedge_i
  \accessible(y_i)$\hfill\null\\[.2em]
Splitting up the heads of rules, we can replace the above by:

\begin{itemize}
\item (Truncated Accessibility):\\$\left(\bigwedge_i \accessible(x_i)\right) \wedge
  R(\vec x, \vec y) \rightarrow \bigwedge_i
  \accessible(y_i)$;
\item (Transfer): $\left(\bigwedge_i \accessible(x_i)\right) \wedge R(\vec x, \vec y)
  \rightarrow  R'(\vec x, \vec y)$.
\end{itemize}

%
Let $\Delta$ be the TGDs of the first kind:
  they are truncated accessibility axioms that 
  represent the propagation of accessibility facts.
Let $\Sigma''$ be the TGDs of the second kind:
the latter $\Sigma''$ represent the transfer from unprimed to primed facts. 
  We now use Proposition~\ref{prop:linearizeaccessids} on~$\Sigma$, $\Sigma'$,
  and~$\Delta$, to obtain $\incd$s $\Sigma^\lift$ of bounded semi-width that can
  emulate all constraints except $\Sigma''$. We can then extend these
  $\incd$s to also capture the effect of~$\Sigma''$ 
  and show that the resulting $\incd$s still have bounded semi-width. This
  allows us to conclude using Proposition~\ref{prop:semiwidthclassic}.
\end{proof}


